Numerical Differentiation-based Electrophysiology-Aware Adaptive ResNet for Inverse ECG Modeling

Electrocardiographic imaging aims to noninvasively reconstruct the electrical dynamic patterns on the heart surface from body-surface ECG measurements, aiding the mechanistic study of cardiac function. At the core of ECGI lies the inverse ECG problem, a mathematically ill-conditioned challenge where small body measurement errors or noise can lead to significant inaccuracies in the reconstructed heart-surface potentials. %Leveraging a well-developed electrophysiological (EP) model, our previous study developed an EP-informed deep learning framework, demonstrating promising effectiveness in improving cardiac map predictions. To improve the accuracy of ECGI and ensure that cardiac predictions adhere to established physical principles, recent advances have incorporated well-established electrophysiology (EP) laws into their model formulations. However, traditional EP-informed models encounter significant challenges, including overfitting to EP constraints, limitations in network scalability, and suboptimal initialization. These issues compromise prediction accuracy and stability, hindering their effectiveness in practical applications. This highlights the need for an advanced data analytic and predictive tool to achieve reliable cardiac electrodynamic restoration. Here, we present a Numerical Differentiation-based Electrophysiology-Aware Adaptive Residual neural Network (EAND-ARN) for robust inverse ECG modeling. Our method employs numerical differentiation to compute the spatiotemporal derivative, enabling EP constraints to be applied across a local spatiotemporal region, thereby strengthening the overall EP enforcement. Additionally, we design an adaptive residual network to improve gradient flow, enhancing predictive accuracy and mitigating issues with poor initialization. Experimental results show that EAND-ARN significantly outperforms existing methods in current practice.

==> backup/conclusion.tex <==
\section{Conclusion}
In this paper, we introduce a novel GL-PINN methodology for solving the inverse ECG problem. Our framework distinctively combines multiple enhancement strategies to achieve superior predictive performance. The core innovation lies in the integration of physics-based constraints derived from the AP model, which ensures our predictions conform to established cardiac electrodynamic principles. To further enhance the model's capabilities, we incorporate geometric information through two key mechanisms: graph Laplacians that capture the spatial relationships in cardiac structures, and fourth-order numerical differentiation that provides higher accuracy in spatial derivatives computation. A significant technical contribution of our work is the implementation of adaptive residual blocks within the PINN architecture. This enhancement addresses two fundamental challenges in deep PINN training: the vanishing gradient problem and sensitivity to poor initialization. Through extensive experimental analysis, we systematically evaluated various network configurations to determine the optimal architecture. Our investigation focused on two critical parameters: the number of neurons per layer and the quantity of adaptive residual blocks, leading to the identification of an optimal network structure that balances computational efficiency with predictive accuracy. Our comparative analysis demonstrates that our GL-PINN framework achieves markedly improved results compared to contemporary approaches in the field, including Tikh\_2nd, STRE, and EPDL methods. The enhancement in performance is particularly evident in the model's ability to accurately reconstruct heart-surface potentials from body-surface measurements, showing increased stability and reduced sensitivity to measurement noise. These improvements stem from our unique combination of physics-informed constraints, geometric information integration, and adaptive neural architecture. The methodology developed in this study presents new possibilities for solving inverse problems in cardiac electrophysiology. Our GL-PINN framework's success in incorporating both physical laws and geometric constraints suggests potential applications in other biomedical inverse problems where similar principles apply. Future research directions could explore the adaptation of our approach to related challenges in medical imaging and physiological signal processing.

==> backup/discussion.tex <==
\section{Discussion}

==> backup/experiment.tex <==
\section{Experimental Design and Results}
Our proposed PINN framework performance of estimating the HSP from BSP was assessed within the spatiotemporal domain of 3D torso-heart data. The experiment data is obtained from the 2007 PhysioNet Computing in Cardiology Challenge \cite{goldberger_physiobank_2000,dawoud_using_2008}, both HSP and BSP are generated using a two-variable cardiac reaction-diffusion model\cite{wang_physiological-model-constrained_2010}. In the 3D geometry, the heart model is defined by 1094 nodes and 2184 mesh elements, while the body surface model comprises 352 nodes and 677 mesh elements, and the number of discrete time intervals used is 661. This configuration yields our transfer matrix $R$ with dimensions 352 × 1094. The reference HSP $u(s,t)$ with dimensions of 1094 × 661 provides a ground truth to evaluate the inverse ECG reconstruction $\hat{u}(s,t)$ with the same dimension. The BSP data, $y(s,t)$ has dimensions 352 × 661 and is used within the data-driven loss $\mathcal{L}_{\text{D}}$ to optimize the PINN and infer the HSP signal. 

We evaluated the performance of our proposed model and explored how variations in neural network architecture, noise levels, and formation of physics embedding affect prediction accuracy, as illustrated in Figure \ref{fig:fishbone}. Our PINN method is compared with established methods, including Tikhonov second-order (Tikh\_2nd), spatiotemporal regularization (STRE), and physics-constrained deep learning framework (EPDL). We evaluate model performance using three key metrics: Relative Error (RE), Correlation Coefficient (CC), and Mean Squared Error (MSE), defined as:

\begin{align}
    RE &= \frac{\sqrt{\sum_{s,t} |\hat{u}(s,t) - u(s,t)|^2}}{\sqrt{\sum_{s,t} |u(s,t)|^2}}\\
    CC &= \frac{\sum_s (û(s,\cdot) - \bar{û}(s,\cdot))^T(u(s,\cdot) - \bar{u}(s,\cdot))}{\sqrt{\sum_s \|û(s,\cdot) - \bar{û}(s,\cdot)\|^2 \sum_s \|u(s,\cdot) - \bar{u}(s,\cdot)\|^2}}\\
    MSE &= \frac{1}{N} \sum_{s,t} |\hat{u}(s,t) - u(s,t)|^2
\end{align}

where $N$ is the total number of spatiotemporal collocation points,$u(s,t)$ and $\hat{u}(s,t)$ are the reference and estimated HSP signals, and the overbars denote the mean of the respective time series. The $RE$ quantifies the deviation of the estimated signal from the reference, with lower values indicating better accuracy. The $CC$ measures the similarity between the reference and predicted patterns, with a value of 1 representing a perfect match, and 0 means the least similarity. The $MSE$ captures the average squared error between the reference and estimated signals.

Our PINN framework is implemented on our high-performance computing (HPC) cluster using PyTorch. PyTorch is a widely adopted deep learning library based on the Torch library and is renowned for its flexibility and efficiency in various machine learning applications, including natural language processing \cite{damentko_msr66_2023} and computer vision \cite{tian_applying_2021}. It supports multiple computing environments, enabling execution across Central Processing Units (CPUs) and Graphics Processing Units (GPUs) \cite{paszke_pytorch_2019}. HPC systems combine advanced hardware architectures with specialized pre-installed software packages, providing an optimal environment for executing complex neural network computations\cite{pratx_gpu_2011}. In this study, we deploy our PINN on a state-of-the-art HPC system equipped with an AMD EPYC 9454 CPU and NVIDIA A100 GPU. This setup ensures the computational demands of our neural network training with high efficiency and accuracy. The version of the PyTorch library used in this study is 2.4, and the Python version is 3.12. 

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{figures/fishbone.png}
\caption{Experimental design for model performance evaluation}
\label{fig:fishbone}
\end{figure}

In the following experiments, the 10-layer 10-neuron fully connected feed-forward neural network with the EPDL method, which is the current advanced method, will serve as our reference baseline model. Our proposed model with special Laplacian and auto-differentiation is denoted as EAND-ARN\textsubscript{AD}, and the model uses the spatial Laplacian and 4th-ND is denoted as EAND-ARN\textsubscript{ND}. We conducted 70000 iterations for each training process. To account for variations, each model we evaluated was executed six times.

\subsection{Validation of Model Effectiveness}

To validate the effectiveness of our proposed model, we conducted an experiment comparing the performance of different physics awareness methods: EPDL, EAND-ARN\textsubscript{AD}, and EAND-ARN\textsubscript{ND}. In detail, three physics awareness methods are executed on the same neural network structure with the same input data and the same model hyperparameters. For the neural network structure, we use our baseline structure (10 layers and 10 neurons in each layer). And for the model hyperparameters, we set the total number of collocation points $N$ = 50000; noise level $\sigma_{\varepsilon}$ = 0.01, which means adding Gaussian noise $\mathcal{N}(0, \sigma_{\varepsilon}^2)$ to the BSP data; and the physics loss intensity $\lambda$ is set to 0.1.

\begin{figure*}[htp]
\centering
\includegraphics[width=7in]{figures/exp1.png}
\caption{The influence of different models on (a) RE, (b) MSE, and (c) CC.}
\label{fig:exp1}
\end{figure*}

The results in figure \ref{fig:exp1} (a-c) illustrate how each method performs in terms of RE, MSE, and CC. EPDL shows the highest RE (0.1435 ± 0.0122), MSE (0.0066 ± 0.0011), and lowest CC (0.9830 ± 0.0028), indicating that incorporating spatial Laplacian can effectively improve the model performance which results in relatively lower errors. On the other hand, both EAND-ARN\textsubscript{AD}, and EAND-ARN\textsubscript{ND} demonstrate better performance, with EAND-ARN\textsubscript{ND} achieving the best results overall: RE of 0.1174 ± 0.0111, MSE of 0.0044 ± 0.0008, and CC of 0.9887 ± 0.0021. The difference between the two models suggests that including 4thh-ND provides a slight but consistent improvement across all metrics. These findings suggest that enhanced integration of heart geometry information can significantly improve model accuracy and robustness. Thus, we choose EAND-ARN\textsubscript{ND} as the primary physics awareness method for our proposed model in the following subsections.

\subsection{Impact of Neural Network Structure on the Prediction
Performance}

In this experiment, our objective is to evaluate the impact of neural network architecture on prediction performance and therefore choose the optimal structure for our inverse ECG problem. Specifically, we focused on exploring the different combinations of the number of neurons in each layer and the number of adaptive residual blocks. The goal is to capture more patterns in the data with deeper networks while carefully managing potential issues like overfitting and vanishing gradients, which ensures the model gains complexity without sacrificing generalization.

\textit{1) Number of Neurons:} Expanding the neurons per layer allows the network to capture more complex patterns and abstractions at each stage of processing. In order to analyze the effect of different numbers of neurons in each hidden layer, We used the same ten layers feedforward neural network with EAND-ARN\textsubscript{ND} as the physics awareness method, and tested three different options for neuron numbers, with 5, 10, and 15 neurons per layer, while maintaining all other hyperparameters constant. The objective was to examine how increasing the network complexity impacts the model’s ability to minimize errors and capture the underlying data structure. By incrementally increasing the number of neurons, we also aimed to quantify the trade-offs between model expressiveness and computational efficiency, thus informing the selection of an optimal network architecture for our inverse ECG problem.

\begin{figure*}[htp]
\centering
\includegraphics[width=7in]{figures/exp2.png}
\caption{The influence of number of neurons on (a) RE, (b) MSE, and (c) CC.}
\label{fig:exp2}
\end{figure*}

As illustrated in Figure \ref{fig:exp2} (a-c), increasing the number of neurons per layer significantly enhances model performance across all metrics. With five neurons, the model exhibits relatively high error rates, with a RE of 0.1658 ± 0.0182 and MSE of 0.0088 ± 0.0019. However, as the neuron count increases to ten and fifteen, we observe a consistent improvement in all performance indicators. The fifteen-neuron configuration achieves the best results, with the lowest RE of 0.1137 ± 0.0137 and MSE of 0.0042 ± 0.0010, while simultaneously maximizing CC at 0.9893 ± 0.0026, compared to 0.9773 ± 0.0048 for the five-neuron setup. These concurrent improvements in RE, MSE, and CC indicate that a higher number of neurons enables the model to better capture the underlying data distribution. However, the marginal gains observed between the ten neurons and fifteen neurons suggest a potential plateau in performance improvement with further complexity increases. Consequently, the fifteen neurons configuration presents an optimal balance between model complexity and performance, and we choose it for subsequent experiments in this study.

\textit{2) Number of Adaptive Residual Blocks:} The implementation of adaptive residual blocks in our PINN enhances the model's ability to capture complex spatiotemporal dependencies in our data. To evaluate the impact of adaptive residual blocks on model performance, we conducted experiments using five different neural network configurations (NN1-NN5), as detailed in table \ref{tab:nnconfig}. These configurations varied in the number of layers, neurons per layer, and the number of residual blocks. NN1 served as our baseline model, which used the EPDL method with 10 layers and 10 neurons in each layer, while NN2 through NN5 employed our EAND-ARN\textsubscript{ND} physics awareness method with 15 neurons per layer, but varied in their structure: NN3 and NN5 incorporated two and three adaptive residual blocks respectively, allowing us to compare the impact of increasing residual blocks. In parallel, NN2 and NN4 were designed without residual blocks but matched the total layer count of NN3 and NN5, respectively, enabling us to isolate the effect of residual blocks while controlling for network depth. This setup allowed us to investigate the effectiveness of residual blocks versus traditional layered structures of equivalent depth. It's important to note that the difference in the total number of layers between some configurations is attributable to the inclusion of residual blocks, as each residual block contains two fully connected layers, thus adding two layers to the network's overall depth. All other model hyperparameters across these five configurations were kept the same as in previous experiments. Through this comprehensive comparison, our aim was to further determine the optimal neural network structure for our model, balancing the benefits of adaptive residual blocks with the overall complexity of the network.

\begin{table}[thb]
    \caption{Neural network configurations\label{tab:nnconfig}}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
        \hline
        & NN1 & NN2 & NN3 & NN4 & NN5 \\ \hline
        Layers & 10 & 7 & 7 & 10 & 10 \\ \hline
        Neurons & 10 & 15 & 15 & 15 & 15 \\ \hline
        Residual Blocks & 0 & 0 & 2 & 0 & 3 \\ \hline
        {Physics Instillation} & EPDL & \multicolumn{4}{c}{EAND-ARN\textsubscript{ND}}\\ \hline
    \end{tabular}
\end{table}

Figure \ref{fig:exp3} (a-c) illustrates the performance of these configurations across the three metrics. The results demonstrate a clear trend of improvement as we introduce and increase the number of adaptive residual blocks. NN1, our baseline model without residual blocks, shows the highest RE (0.1435 ± 0.0122) and MSE (0.0066 ± 0.0011), and the lowest CC (0.9830 ± 0.0028). Comparing NN2 and NN3, which have the same total number of layers but differ in the presence of residual blocks, we observe that NN3 with two residual blocks outperforms NN2 across all metrics (RE: 0.1121 ± 0.0064 vs 0.1250 ± 0.0199, MSE: 0.0040 ± 0.0005 vs 0.0051 ± 0.0017, CC: 0.9897 ± 0.0012 vs 0.9869 ± 0.0043). Similarly, NN5 with three residual blocks shows superior performance compared to NN4 with the same total layers but no residual blocks (RE: 0.0992 ± 0.0062 vs 0.1137 ± 0.0137, MSE: 0.0031 ± 0.0004 vs 0.0042 ± 0.0010, CC: 0.9919 ± 0.0010 vs 0.9893 ± 0.0026). As we progress from NN3 to NN5, increasing the number of residual blocks from two to three, we observe a further consistent decrease in RE and MSE, coupled with an increase in CC. Notably, NN5 achieves the best performance across all metrics. This substantial improvement over the baseline (31\% reduction in RE, 53\% reduction in MSE, and 0.9\% increase in CC) underscores the efficacy of adaptive residual blocks in enhancing model performance. The consistent trend across all three metrics suggests that the introduction of adaptive residual blocks enables the network to capture more complex patterns and learn richer representations, effectively addressing the limitations of traditional FNNs in solving inverse ECG problems. 

\begin{figure*}[!t]
\centering
\includegraphics[width=7in]{figures/exp3.png}
\caption{The influence of different neural network structures on (a) RE, (b) MSE, and (c) CC.}
\label{fig:exp3}
\end{figure*}

To evaluate the effectiveness of adaptive residual blocks in improving the bad initialization problem in PINNs, we also conducted an experiment comparing the initialization performance across our five neural network configurations. We defined bad initialization as instances where the total loss $\mathcal{L}$ exceeded 1.5 during the first 300 iterations. To ensure statistical robustness and minimize the impact of randomness, we ran each configuration 30 times, in line with the central limit theorem. Table \ref{tab:badinitial} presents the results of this experiment. Notably, the configurations with adaptive residual blocks (NN3 and NN5) demonstrated significantly lower bad initialization rates compared to their counterparts without residual blocks. NN3, with two residual blocks, reduced the bad initialization rate to 13.33\% from 76.67\% in NN2, while NN5, with three residual blocks, achieved a 20.00\% rate compared to 60.00\% in NN4. These results strongly indicate that adaptive residual blocks substantially improve the initialization stability of PINNs, potentially by allowing the network to start with a simpler structure and gradually increase complexity during training.

\begin{table}[hb]
    \caption{Comparison of bad initialization rates across different neural network models \label{tab:badinitial}}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
        \hline
        & NN1 & NN2 & NN3 & NN4 & NN5 \\ \hline
        Bad Initialization & 16 & 23 & 4 & 18 & 6 \\ \hline
        Total Runtime & 30 & 30 & 30 & 30 & 30 \\ \hline
        Bad Initial Rate & 53.33\% & 76.67\% & 13.33\% & 60.00\% & 20.00\% \\ \hline
    \end{tabular}
\end{table}

The above results validate our approach of using adaptive residual blocks to mitigate poor initialization issues and improve the network's ability to utilize increased depth and complexity effectively, both when compared to networks without residual blocks and when increasing the number of residual blocks. Therefore, we selected NN5 – consisting of 10 layers, 15 neurons per layer, and 3 adaptive residual blocks – as our optimal network structure for subsequent comparisons in this study.

\subsection{Comparison Study with Different Models}

In this experiment, we conducted a comprehensive comparison between our proposed EAND-ARN\textsubscript{ND} approach and three widely used models: Tikh\_2nd, STRE, and EPDL, which were used as benchmarks. Based on the results from previous experiments, we configured our EAND-ARN\textsubscript{ND} model as an FNN with three adaptive residual blocks, 10 layers, and 15 neurons per layer. Our analysis focused on the performance of these methods across various noise levels ($\sigma_{\varepsilon}$ = 0.01, 0.05, and 0.1). Figure \ref{fig:exp4} presents a detailed comparison of RE, MSE, and CC for all four methods under different noise conditions. 

\begin{figure*}[!t]
\centering
\includegraphics[width=5.5in]{figures/exp4.png}
\caption{The comparison of methods (i.e., Tikh\_2nd, STRE, EPDL, and EAND-ARN) on (a) RE, (b) MSE, and (c) CC under different BSP noise levels (0.01, 0.05, and 0.1)}
\label{fig:exp4}
\end{figure*}

Our proposed model consistently demonstrates superior performance compared to other benchmark methods for all noise levels, achieving the lowest MSE and RE values while maintaining the highest CC scores. For instance, at $\sigma_{\varepsilon}$ = 0.01, EAND-ARN\textsubscript{ND} achieved an RE of 0.0992 ± 6.16e-03, an MSE of 0.0031 ± 3.88e-04, and a CC of 0.9830 ± 2.78e-03, outperforming all other models. In contrast, the Tikh\_2nd method struggled with accurately reconstructing the HSP, producing the highest MSE and RE values. At $\sigma_{\varepsilon}$ = 0.1, for example, Tikh\_2nd exhibited an MSE of 0.0681 ± 6.19e-04 and an RE of 0.4625 ± 1.31e-03, significantly higher than the other methods. Both STRE and EPDL showed improvements over Tikh\_2nd, demonstrating the benefits of incorporating additional regularizations and constraints into the models. The performance of our model indicates the successful integration of physical prior knowledge and spatial constraints, resulting in enhanced accuracy. Meanwhile, as the increases of noise level from 0.01 to 0.1, we observe a consistent upward trend in both MSE and RE for all methods. However, the magnitude of this increase varies significantly among the techniques. While all the other three methods show a reasonable increase, the Tikh\_2nd method has the highest sensitivity to noise, with a 73.48\% increase in RE and a 202.67\% increase in MSE. The CC metric shows a similar pattern. This result reveals the effectiveness and robustness of physics-informed approaches and demonstrates our model correctly leveraging physical prior information and maintaining robust performance across varying noise levels.

\begin{figure*}[htbp]
\centering
\includegraphics[width=6in]{figures/exp5.png}
\caption{Spatial visualization of (a)Reference HSP, Different methods (Tikh\_2nd, STRE, EPDL, and EAND-ARN) estimated HSP with noise level (b) 0.01, (c) 0.05, and (d) 0.1 at t = 300}
\label{fig:exp5}
\end{figure*}

\begin{figure*}[htbp]
\centering
\includegraphics[width=6in]{figures/exp6.png}
\caption{Spatial visualization of (a)Reference HSP, Different methods (Tikh\_2nd, STRE, EPDL, and EAND-ARN) estimated HSP with noise level (b) 0.01, (c) 0.05, and (d) 0.1 at t = 320 in another angle}
\label{fig:exp6}
\end{figure*}

Figures \ref{fig:exp5} and \ref{fig:exp6} show the spatial visualization of the estimated HSP distributions on the heart surface at selected time points (300 and 320) with anterior view and posterior view, illustrating a complete depolarization process from the apex to the base. In both figures, panel (a) represents the actual potential distribution as the reference, while panels (b-d) depict the predicted HSP distributions under varying noise levels ($\sigma_{\varepsilon} = 0.01$ for b, $0.05$ for c, and $0.1$ for d). The quantitative metrics highlight that EAND-ARN\textsubscript{ND} demonstrates superior accuracy. At the same time, Tikh\_2nd and STRE show more pronounced deviations, especially at higher noise levels. Specifically, at $\sigma_{\varepsilon}$ = 0.1, EAND-ARN\textsubscript{ND} achieved the best results with RE of 0.0895, MSE of 0.0025 and CC of 0.9935. In contrast, EPDL’s performance under the same noise conditions is slightly inferior, with RE, MSE, and CC values of 0.1446, 0.0066, and 0.9829, respectively. STRE shows more discrepancy with results of 0.2490, 0.0197, and 0.9481, while Tikh\_2nd exhibits the largest errors, with an RE of 0.5569, MSE of 0.0983, and CC of 0.7501. Comparing the color patterns of each model to the reference, EAND-ARN\textsubscript{ND} consistently provides the closest approximation to the true potential distribution under all noise conditions. Although EPDL achieves comparable results, the posterior view reveals that EAND-ARN\textsubscript{ND} achieves a marked improvement in prediction accuracy, particularly in the base of the heart region. In this area, EAND-ARN\textsubscript{ND} demonstrates a smoother, more precise representation of the unactivated potential compared to EPDL, which exhibits less continuity and detail. This enhanced accuracy in EAND-ARN\textsubscript{ND} is supported by its consistently lower RE and MSE values and higher CC scores across all noise levels, indicating that EAND-ARN\textsubscript{ND} not only aligns closely with the actual distribution but also captures fine-scale variations more effectively. Both the quantitative metrics and spatial visualizations exhibit that our model achieves the highest prediction fidelity and effectively preserves spatial detail in high-noise scenarios, particularly around critical areas such as the heart’s base.

\begin{figure*}[!t]
\centering
\includegraphics[width=7in]{figures/exp7.png}
\caption{The comparison of Reference HSP and different methods (Tikh\_2nd, STRE, EPDL, and EAND-ARN) estimated HSP evolvement over time at a specific spatial location with noise level (a) 0.01, (b) 0.05, and (c) 0.1}
\label{fig:exp7}
\end{figure*}

Figure \ref{fig:exp7} (a-c) presents the temporal evolution of the estimated HSP using four methods at a specific spatial location under varying noise conditions ($\sigma_{\varepsilon}$ = 0.01 for b, 0.05 for c, and 0.1 for d). The results indicate that EAND-ARN\textsubscript{ND} and EPDL achieve high accuracy, producing estimates closely aligned with the true HSP, while demonstrating noise robustness by effectively smoothing out noisy fluctuations. A detailed zoom-in view for the time interval 190-290 is shown, which further highlights that EAND-ARN\textsubscript{ND} outperforms the EPDL, particularly during the upstroke phase of the heartbeat. In contrast, Tikh\_2nd shows substantial noise-induced oscillations and low accuracy in reconstructing the HSP. Although the STRE method delivers a smoother result through temporal regularization, it still deviates from the true HSP. By integrating physics prior knowledge of cardiac electrodynamics, EPDL and EAND-ARN\textsubscript{ND} provide more accurate estimations, with EAND-ARN\textsubscript{ND} performing best due to its additional consideration of geometric information in the modeling process.

\subsection{Impact of Physics Loss Intensity on the Prediction Performance}

The physics loss intensity, represented by $\lambda$ plays a crucial role in balancing the data-driven loss $\mathcal{L}_{\text{D}}$ with the EP awareness loss $\mathcal{L}_{\text{Ep}}$. Our study examined the impact of this hyperparameter on prediction performance by testing $\lambda$ values of 0.05, 0.1, 0.3, 0.5, and 0.7. The results presented in table \ref{tab:physics} indicate that varying the intensity of the physics loss parameter $\lambda$ affects model performance metrics, including RE, CC, and MSE. When $\lambda$ is set to 0.1, the model achieves the lowest RE of $0.0992 \pm 0.0062$ and the highest CC of $0.9919 \pm 0.0010$. Based on the result, only $\lambda$ = 0.1 yielded favorable results, allowing for error reduction and convergence of the loss function. In contrast, other $\lambda$ values resulted in less favorable performance, where both error and loss failed to decrease effectively. This suggests that the influence of physics constraints must be carefully calibrated. And $\lambda$ = 0.1 proved to be the most effective in our experiments, indicating that a subtle integration of physical laws enhances the model's performance without overwhelming the data-driven learning process.

\begin{table}[thb]
    \caption{Model performance under different physics loss intensities\label{tab:physics}}
    \centering
    \begin{tabular}{c|c|c|c}
        \hline
        \lambda & RE & CC & MSE \\ \hline
        $0.05$ & $0.1012 \pm 0.0089$ & $0.9916 \pm 0.0015$ & $0.0033 \pm 0.0006$ \\ \hline
        $0.1$  & $0.0992 \pm 0.0062$ & $0.9919 \pm 0.0010$ & $0.0031 \pm 0.0004$ \\ \hline
        $0.3$  & $0.1256 \pm 0.0021$ & $0.9871 \pm 0.0004$ & $0.0050 \pm 0.0002$ \\ \hline
        $0.5$  & $0.1252 \pm 0.0035$ & $0.9872 \pm 0.0007$ & $0.0050 \pm 0.0003$ \\ \hline
        $0.7$  & $0.1279 \pm 0.0005$ & $0.9866 \pm 0.0001$ & $0.0052 \pm 0.0001$ \\
    \hline
    \end{tabular}
\end{table}

==> backup/introduction.tex <==
\section{Introduction}
The advancement of medical sensing and imaging technologies has created a data-rich environment, enabling smart health solutions that support more precise diagnostics and personalized treatment approaches. Among these advances, electrocardiography (ECG) stands out as a critical tool for non-invasive cardiac monitoring and diagnostics. It measures electrical signals on the body surface originating from the epicardium, capturing the spatiotemporal patterns that reflect the heart’s rhythmic activity. %Clinically, the twelve-lead ECG is widely used to capture multi-angle views of cardiac electrodynamics by recording electrical signals from different regions of the body. While the traditional twelve-lead ECG \cite{yang_spatiotemporal_2013} is effective for disease detection, it does not capture sufficient detail to provide comprehensive information about the heart's electrical distribution and spatial dynamics. This limitation hinders precise localization of diseased origins on the heart's surface. To address this, Body Surface Potential Mapping (BSPM) extends ECG's utility by using a higher density of sensors across the torso, enabling a more accurate understanding of cardiac electrical activity and potentially pinpointing specific areas of dysfunction \cite{horacek_optimal_2001,bond_xml_2009,lacroix_evaluation_1991,rudy_noninvasive_1999,zhu_optimal_2019,chen_sparse_2016}. 
%Clinically, the twelve-lead ECG is widely used to capture multi-angle views of cardiac electrodynamics by recording electrical signals from different regions of the body. 
While the traditional twelve-lead ECG \cite{yang_spatiotemporal_2013} is effective for disease detection, it does not capture sufficient detail to provide comprehensive information about the heart's electrical distribution and spatial dynamics. %This limitation hinders precise localization of diseased origins on the heart's surface. 
To address this, Body Surface Potential Mapping (BSPM) extends ECG's utility by using a higher density of sensors across the torso, enabling a more accurate understanding of cardiac electrical activity and potentially pinpointing specific areas of dysfunction \cite{horacek_optimal_2001,bond_xml_2009,lacroix_evaluation_1991,rudy_noninvasive_1999,zhu_optimal_2019,chen_sparse_2016}. 




%The heart chambers produce electrical waves through depolarization and repolarization during contraction and relaxation, creating distinct patterns of cardiac activity across spatiotemporal domains \cite{somani_deep_2021,oster_electrocardiographic_1998}. Standard ECG signals are often recorded through the Twelve-lead system, with a ten-electrodes configuration, which positions across specific regions on the torso and limbs to infer cardiac electrodynamics\cite{yang_spatiotemporal_2013}. The limited number of electrodes in traditional ECG systems (e.g., 12-lead ECG) restricted the capture of fine-grained cardiac electrodynamics throughout the entire heart, resulting in relatively low spatial resolution and potentially missing crucial cardiac electrical information \cite{herring_ecg_2006}. To address this limitation, body surface potential mapping (BSPM) has emerged as an advanced solution, utilizing an expanded array of electrodes (e.g., Dalhousie Standard Torson 120 configuration) to yield high-resolution spatiotemporal body signal maps that reflect the cardiac behavior. This enhanced measurement approach enables detailed mapping and localization of cardiac activity\cite{horacek_optimal_2001,bond_xml_2009,lacroix_evaluation_1991,rudy_noninvasive_1999,zhu_optimal_2019,chen_sparse_2016}.

While high-resolution BSPM provides comprehensive spatiotemporal information about cardiac electrical activity, translating this surface data into meaningful insights about the underlying cardiac electrodynamics requires solving the inverse ECG problem \cite{rudy_noninvasive_1999,oster_noninvasive_1997,gulrajani_forward_1998,yao_mesh_2016,yao_spatiotemporal_2020,macleod_recent_1998}. However, this problem is inherently ill-posed, meaning that small errors or noise in the body measurements can lead to disproportionately large errors in the heart solution\cite{patel_solution_2022}. This challenge underscores the need for robust data analytics tools that can effectively handle the complex data structure and  manage measurement noise, providing accurate heart signal reconstruction.  


%These reconstructions offer essential insights into cardiac function, supporting accurate heart condition diagnosis, disease monitoring, and personalized therapeutic strategies \cite{rudy_noninvasive_1999,oster_noninvasive_1997,gulrajani_forward_1998,yao_mesh_2016,yao_spatiotemporal_2020,macleod_recent_1998}. However, because HSP and BSPM are measured on different surfaces with different resolutions and geometries, the inverse ECG problem is inherently ill-posed, which presents significant challenges \cite{patel_solution_2022}. Multiple solutions to the problem may exist, and small measurement errors can result in dramatically different reconstructions. Also, the computational demands of processing high-resolution BSPM data are substantial, particularly given the complex geometrical, mechanical, and electrical properties of the heart. Furthermore, when cardiac electrical signals propagate from the heart to the body surface, their spatiotemporal patterns become attenuated and distorted, making it challenging to identify local cardiac abnormalities accurately. These challenges underscore the need for more sophisticated methodological approaches, as improved reconstruction accuracy directly enhances diagnostic capabilities and patient care outcomes.

%To solve the inverse ECG problem and produce an accurate and robust solution, significant effort has been invested by the research community. A key area of investigation has focused on regularization techniques, including spatial regularization approaches (e.g., Tikhonov regularization) and spatiotemporal regularization (e.g., STRE) \cite{ramanathan_noninvasive_2004,tikhonov_solutions_1977,yao_physics-driven_2016}. Although STRE improves Tikhonov regularization by incorporating temporal continuity for a more dynamic representation of cardiac events, the data-driven nature of both methods presents limitations. These regularization techniques often struggle to process complex spatiotemporal data effectively, leading to compromised reconstruction accuracy. 

 Statistical regularization is a commonly used approach to stabilize the reconstruction of cardiac electrodynamics by suppressing unreliable variations in heart signals. For example, Tikhonov regularization\cite{ramanathan_noninvasive_2004,tikhonov_solutions_1977}, which applies a penalty with the L2 norm, promotes spatial smoothness in the reconstructed heart signal by reducing high-frequency noise. To further enhance coherence across time, spatiotemporal regularization (STRE) methods \cite{yao_physics-driven_2016} have been developed, promoting not only spatial smoothness but also temporal continuity. However, these statistical regularization methods focus primarily on matching heart predictions with sensor observations, and their expressiveness is limited with oversimplified model structures. Consequently, they often yield skewed and noisy cardiac solutions. % that fail to adhere to well-established electrophysiological (EP) principles.

In cardiac research, several phenomenological models have been developed to characterize the propagation of electrical waves across the heart, providing valuable physical insights into the mechanisms underlying cardiac function.\cite{camara_inter-model_2011,sermesant_electromechanical_2006}. Solving these models merely provides theoretical representations of heart dynamics, without the ability to incorporate real-world sensing data. Consequently, these well-established EP rules are often overlooked in the traditional regularization approach. %, limiting the predictive accuracy. 
To leverage this valuable prior knowledge of dynamic electrical patterns, recent research has advanced inverse ECG modeling by integrating EP models into deep learning frameworks. Specifically, the EP laws are embedded into the loss function in a residual format alongside the sensor observation loss, ensuring that the model output—cardiac electrodynamics—not only aligns with body ECG observations but also adheres to established EP rules. This integration allows the EP models to inform cardiac predictions, enhancing the physiological accuracy and robustness of the reconstructed cardiac activity. \cite{xie_physics-constrained_2023}.

%Despite the aforementioned advances,  the EP-constrained Deep Learning (EPDL) model is still facing challenges. 


%Recently research has focused on better embedding physics into the model while effectively balancing physical principles with data-driven adaptability. Probabilistic estimation approaches, particularly state-space models \cite{wang_physiological-model-constrained_2010}, exemplify this integration by representing cardiac electrical activity through physics-informed transition matrices and employing Kalman filtering for dynamic updates. However, this model requires initial cardiac conditions, which are often unavailable or challenging to measure non-invasively.   %demonstrated the potential of incorporating physics knowledge into deep learning through Electrophysiology (EP) awareness loss, successfully improving solution stability and accuracy. 
%Despite the advances, the EPDL model's oversimplified neural network structure and loose physics constraints indicate the potential for further improvement in prediction accuracy. Based on our previous work, this paper introduces a novel GL-PINN framework, effectively improves the reconstruction of HSP across various noise levels. The summary of our key contributions is as follows:


Despite the aforementioned advances, the EP-constrained Deep Learning (EPDL) model still faces significant challenges. The first challenge arises from the depth limitations of neural networks in the EPDL model. 
While increasing network depth could theoretically enhance feature expressiveness and nonlinear feature extraction, prior work often resorts to smaller, shallower networks to avoid issues like network degradation and ineffective network scaling. Furthermore, the conventional feedforward architecture in traditional EPDL models may introduce initialization challenges, making the network more prone to gradient explosion or vanishing. These issues ultimately undermine the model’s predictive accuracy and stability, limiting the effectiveness of deeper architectures in capturing complex cardiac dynamics. In addition, the EP-informed framework requires a large corpus of spatiotemporal collocation points to enforce the imposed EP rules during training, which introduces a substantial computational burden. The automatic differentiation (AD) calculates the derivatives in the EP model at individual spatiotemporal points, which does not consider neighboring relationships. This isolated differentiation approach may limit the model's ability to capture coherent spatiotemporal dynamics, leading to suboptimal predictive accuracy. To address these limitations, we propose a Numerical Differentiation-based EP-aware Adaptive Residual Network (EAND-ARN) to improve the accuracy of inverse ECG solutions. Our major contributions are: 

1)We introduce an adaptive ResNet structure that mitigates initialization pathology, enabling stable and efficient scaling of the neural network architecture design for accurate cardiac predictions. 
Our proposed framework enhances traditional residual connections by introducing a trainable parameter constrained between 0 and 1. This setup addresses fundamental challenges in training significantly deepened EPDL networks. Moreover, this structure improves explainability by indicating what percentage of the output is directly inherited from the input through the adaptive residual block versus what portion is newly learned. Moreover, it effectively mitigates the poor initialization problem that exists in the original EPDL model, leading to more stable and accurate training outcomes.

%We address the optimization challenges associated with PINNs by leveraging the adaptive ResNet architecture. Our proposed framework transforms traditional skip connections into adaptive residual blocks with trainable intensities, allowing dynamic control of information flow between layers. This architectural innovation not only mitigates vanishing gradients and initialization sensitivity but also enhances model interpretability through quantifiable layer contributions. The resulting deeper network structure effectively captures complex cardiac spatiotemporal patterns while maintaining robust training dynamics.

2) We innovatively incorporate numerical differentiation to calculate derivatives and the Laplacian within the EP residual, enhancing EP enforcement. To calculate the spatial Laplacian for a 3D heart geometry, we leverage a Laplacian operator derived from the spatial geometric relationships among neighboring nodes. Additionally, we utilize a fourth-order Taylor expansion to compute temporal derivatives based on neighboring points. This approach enables the EP constraint to operate not only on individual instance but also to account for spatiotemporal locality, improving the coherence and accuracy of the model's predictions across space and time.

%We incorporate two numerical differentiation techniques on both spatial and temporal domain into our EP awareness loss, providing additional geometry information. The spatial Laplacian encodes the inherent geometric relationships across the heart surface, while fourth-order differentiation schemes ensure accurate spatial gradient computations. By embedding these constraints, our model enhanced the ability to capture the structural characteristics of cardiac electrical propagation, leading to better preservation of spatiotemporal patterns.

Through experimental validation, our EAND-ARN framework demonstrates superior performance in inverse ECG reconstruction compared to state-of-the-art methods. Our results show significant improvements in reconstruction accuracy across different noise levels, marking an important advancement in precision cardiology and clinical applications.

The remainder of this paper is organized as follows: Section II provides a literature review of relative techniques to solve inverse ECG problems. Section III presents our EAND-ARN methodology, detailing the mathematical formulation of EAND-ARN architecture. Section IV provides experimental results and comparative performance analysis. Finally, Section V concludes with a summary of our findings.




==> backup/literature.tex <==
\section{Literature Review}
\subsection{Traditional Methods for Solving Inverse ECG Problem}
The inverse ECG problem aims to non-invasively reconstruct electrical activity within the heart using body surface sensor data, which is vital for the accurate diagnosis and assessment of heart conditions and is also important for the development of cardiac disorder treatments. This process applies an approximation of Maxwell's equations to the electromagnetic field between the heart and torso to define the connection between ECG data and cardiac electrical excitation. By numerically solving these equations on heart-torso models, a linear relationship between the body surface potential map (BSPM), denoted as $ y(s, t)$, and the heart surface potential (HSP), represented as $u(s, t)$, can be derived as: $y(s, t) = R u(s, t) +\epsilon$, where $s$ and $t$ represent the position and time instant, the transfer matrix $R$ is determined using the Divergence Theorem and Green’s Second Identity, and $\epsilon$ denotes the noise term that captures errors from both measurement and modeling \cite{yao_physics-driven_2016,karoui_evaluation_2018}. Due to the dimensional mismatch between the large number of unknown electrical potentials on the heart surface and the limited number of body surface measurements we can practically obtain, the inverse ECG problem is inherently ill-posed. This mismatch manifests in the transfer matrix $R$, which suffers from rank deficiency and a high condition number. Even minor uncertainties in the body surface measurements, such as noise, measurement errors, and model approximations, will be dramatically amplified when solving for the HSP \cite{patel_solution_2022}. Stabilizing this inverse ECG solution is crucial, as it is essential for clinical applications, including early diagnosis of cardiac arrhythmias, localization of irregular heart rhythms, non-invasive cardiac electrical mapping, and guidance for catheter ablation procedures.

Traditionally, a lot of existing literature was focused on applying regularization methods on the cardiac spatiotemporal data to stabilize the inverse ECG problem. One of the popular choices is spatial regularization, which introduces spatial constraints to improve the reconstruction of HSP \cite{figuera_regularization_2016,rodrigo_solving_2018}. L1-norm regularization, which promotes sparsity by penalizing the absolute values of the model's coefficients. This approach is particularly effective at identifying and preserving dominant features while suppressing noise by encouraging sparse solutions \cite{ghosh_application_2009}. Tikhonov regularization (both zero-order and first-order), stabilizes the reconstruction by introducing L2-norm spatial constraints that minimize abrupt spatial variations and promote smoothness across the HSP. This is achieved through optimizing the objective function:
\begin{align*}
    \min_{u(s,t)} {|y(s,t) - Ru(s,t)|_2^2 + \lambda_{Tikh}^2|\Gamma u(s,t)|_2^2}
\end{align*}
where $\lambda_{Tikh}$ controls regularization strength and $\Gamma$ serves as either an identity matrix (zero-order) or a gradient operator (first-order) to penalize solution magnitude or spatial variations respectively \cite{tikhonov_solutions_1977,wang_resolution_2010,kara_ecg_2019,bear_impact_2021,schuler_reducing_2022,rababah_effect_2021}. However, both L1 and Tikhonov regularization methods have significant limitations. They tend to oversimplify the model by omitting the influence of smaller, more nuanced patterns in the data, leading to reduced model capability. Moreover, they process each time instant independently, failing to capture complex temporal dependencies in cardiac electrical activity. To better incorporate temporal information, spatiotemporal regularization techniques were developed. Messnarz et al. \cite{messnarz_new_2004} developed a spatiotemporal approach that combines first-order Tikhonov regularization in the spatial domain with a temporal constraint that assumes non-decreasing potential values during the depolarization phase. This method improves reconstruction stability but has limitations in handling abnormal cardiac conditions where the non-decreasing assumption may not hold. Yao et al.  \cite{yao_physics-driven_2016} proposed the STRE model, which introduces a spatial Laplacian operator to handle approximation errors through spatial correlations on complex geometries, while simultaneously applying temporal constraints over specified time windows to increase model robustness to measurement noise. As STRE considers the relationships between adjacent time points within a defined window, it achieves better prediction accuracy by capturing both spatial and temporal characteristics of cardiac electrical propagation. However, STRE methods also face some challenges. They are computationally intensive due to processing multiple time windows simultaneously, and require specialized optimization techniques like the dipole multiplicative update algorithm to solve their complex objective functions, making implementation more challenging in practice.

Beyond these approaches, researchers have explored various other methods to enhance inverse ECG reconstruction. Wang et al. \cite{wang_physiological-model-constrained_2010} developed a physiological-model-constrained Kalman filter (P-KF), reformulates the cardiac system as a high-dimensional stochastic state-space model, reconstructed heart potential distributions using the unscented Kalman filter. However, it faces computational challenges due to large matrix operations, and it also heavily relies on unrealistic initial conditions. Despite these advances, there remains a significant gap in leveraging modern machine learning techniques, especially deep neural networks, that can effectively integrate physics-based constraints and produce more accurate inverse ECG modeling.

\subsection{Physics-informed Neural Networks (PINNs)}

Physics-informed neural networks (PINNs) have emerged as a powerful framework for solving partial differential equations (PDEs) by training neural networks to adhere to physical laws. It is a mesh-free method, so it offers the flexibility to allow on-demand solutions after the training phase\cite{cuomo_scientific_2022}. As the physics prior knowledge guides the learning process, it also offers better data efficiency compared to regular neural networks\cite{farea_understanding_2024}. Since their introduction by Raissi et al. \cite{raissi_physics-informed_2019}, PINNs have been successfully applied across various domains, including material designing \cite{chen_physics-informed_2020,liu_multi-fidelity_2019}, fluid dynamics\cite{cai_physics-informed_2021}, quantum mechanics\cite{camporeale_data-driven_2022}, and elastodynamic\cite{rao_physics-informed_2021}. 

Various research has been done using PINN in cardiac electrophysiology. Sahli et al. \cite{sahli_costabal_physics-informed_2020} employed PINNs to solve the eikonal equation for generating high-resolution activation time maps. Martin et al. \cite{herrero_martin_ep-pinns_2022} demonstrated the capability of PINNs to reconstruct action potential propagation and estimate electrophysiological parameters in 1D and 2D scenarios using the Aliev-Panfilov (AP) model. However, these studies are limited by their lack of application to 3D cardiac geometry. Ye et al. \cite{ye_spatial-temporally_2023} presented an adaptive PINN framework for bi-ventricular electrophysiological processes simulation, they introduces weak-form PDE residuals to address complex 3D geometries and employs spatiotemporal weighting alongside a sequential learning strategy to achieve accurate PDE solutions over segmented time domains. Xie et al. \cite{xie_physics-constrained_2023} proposed a EPDL framework which integrats the AP model into deep neural networks to reconstruct cardiac surface potentials from 3D body surface potential spatiotemporal data, showing superior robustness and noise resistance compared to existing methods of solving inverse ECG problems.

However, traditional PINN approaches face some theoretical difficulties. For example, poor initialization of PINNs can destabilize training, cause convergence issue, and produce inconsistent solutions or failure to satisfy boundary conditions \cite{mo_data-driven_2022,cuomo_scientific_2022}. Moreover, conventional PINN architectures suffer from gradient vanishing issues and degraded performance with increasing network depth, limiting their ability to capture complex spatiotemporal dynamics in deep architectures \cite{berg_unified_2018}. These challenges underscore the need for novel neural network architectures specifically designed to overcome these limitations of PINNs.

Furthermore, most existing PINN implementations rely on automatic differentiation (AD), which computes exact derivatives through chain rule during backpropagation \cite{baydin_automatic_2018}. Although AD provides exact gradients, this approach can lead to nonphysical solutions by perfectly satisfying equations at isolated collocation points while missing broader spatial patterns \cite{chiu_can-pinn_2022}. When neural networks are heavily over-parameterized, AD-formulated loss functions often become under-constrained optimization problems \cite{sirignano_dgm_2018}. This limitation is particularly problematic for cardiac applications where electrical propagation depends heavily on the heart's complex geometry. In contrast, numerical differentiation (ND) approximates derivatives using neighboring points based on Taylor series expansions\cite{anderson_computational_2020}, ND can address the limit by naturally coupling neighboring points through local support regions, allowing PINNs to learn coherent patterns even with sparse sampling by modulating gradient behaviors at piecewise local regions rather than at isolated points \cite{chiu_can-pinn_2022}.


==> backup/methodology.tex <==
\section{Methodology}
\subsection{Cardiac Electrophysiology Model}
Cardiac electrophysiology plays a pivotal role in understanding the dynamics of electrical signal propagation in the heart.  %However, due to its structural complexity, many simplified models have been developed in order to make it computationally feasible while providing the necessary details of cardiac functions \cite{camara_inter-model_2011,sermesant_electromechanical_2006}. In our research, 
To achieve a balance between computational efficiency and the ability to study critical cardiac dynamics, we adopted the Aliev-Panfilov (AP) model \cite{aliev_simple_1996}, a commonly used framework for simulating cardiac excitation and signal propagation in cardiac tissue. The AP model is defined by the following set of partial differential equations: 

\begin{align}
\label{cem}
    \frac{\partial u}{\partial t} &= \nabla \cdot (D\nabla u) u + k u (u - a)(1 - u) - u v  \label{AP}\\
    \frac{\partial v}{\partial t} &= \xi(u, v)(-v - k u (u - a - 1)) \\
    \mathbf{n} \cdot \nabla u \big|_{\Gamma_H} &= 0 \label{bd}
\end{align}
where $u$ represents the normalized HSP, and $v$ denotes the recovery current that governs the local depolarization of membrane potential. The coupling interaction between $u$ and $v$ is characterized by $\xi(u, v) =  e_0 + \mu_1 v / (u + \mu_2)$. $D$ is the diffusion coefficient that controls the conduction velocity, $k$ is the repolarization constant that controls the shape of the action potential, and $a$ controls the tissue excitability. In this study, we assume the homogeneity of the heart tissue, which allows us to simplify the diffusion term as $\nabla \cdot (D\nabla u)=D\Delta u $, where $\Delta u$ represents the Laplacian of the HSP $u$. these parameter values are set based on existing literature \cite{aliev_simple_1996}: $a = 0.1$, $D = 10$, $k = 8$, $e_0 = 0.002$, and $\mu_1 = \mu_2 = 0.3$. Eq. \ref{bd} is a Neumann boundary condition that ensures there is no flux of the electrical potential $u$ across the heart boundary $\Gamma_H$, where $n$ is The unit normal vector to the boundary $\Gamma_H$. The AP model defined in Eqs. \ref{AP}-\ref{bd}, will be integrated into a deep learning framework to further enhance the HSP prediction, ensuring that the results are grounded in physical significance.
%where $u$ and $v$ represent the normalized HSP and the recovery current that regulates the local depolarization dynamics of the cardiac electrical potential, $\Gamma_H$ and $\mathbf{n}$ represent the heart boundary and its surface normal accordingly. Other constants are defined as follows: $\varepsilon(u,v) = e_0 + \mu_1 v / (u + \mu_2)$ shows the interaction between $u$ and $v$, $D$ is the diffusion conductivity, $k_r$ is the repolarization constant, and $e_0$ shows the tissue excitability. In our study, these parameter values are set based on existing literature \cite{aliev_simple_1996}: $a = 0.1$, $D = 10$, $k_r = 8$, $e_0 = 0.002$, and $\mu_1 = \mu_2 = 0.3$. The AP model is defined by a system of differential equations involving the HSP and recovery current, and is further constrained using a no-flux boundary condition to ensure the electric current is confined within the heart boundary. To increase our neural network’s robustness and accuracy, the AP model was employed in our study to provide constraints for the training process of the network.

\subsection{Adaptive Residual Neural Networks}
Multilayer perceptrons (MLPs) are the most commonly used neural network architecture in PINNs. \cite{k_review_2014,abiodun_state---art_2018,wang_deep_2018}. A Multilayer Perceptron (MLP) is a type of artificial neural network composed of an input layer, one or more hidden layers, and an output layer, where each layer is fully connected to the next. Each neuron in an MLP processes a weighted sum of its inputs and passes the result through an activation function, typically non-linear, enabling the network to learn complex patterns and approximate highly non-linear functions. The output of the $l$-th layer can be mathematically expressed in its general form as:

%A typical MLP consists of an input layer, several hidden layers, and an output layer, all connected in a sequential manner. Within the FNNs, the information moves only in one direction—from the input layer through one or more hidden layers to the output layer. There are no cycles or loops in the network, making it a direct forward mapping from inputs to outputs. In the hidden layers, each neuron's value is computed as the weighted sum of the outputs from the preceding layer, followed by the activation function to produce its output. The network learns by adjusting these weights using backpropagation to minimize the loss function. The general form of the output for a single layer can be expressed mathematically as:

\begin{equation}
    \mathbf{x}^{(l)} = \sigma(\mathbf{W}^{(l)} \mathbf{x}^{(l-1)} + \mathbf{b}^{(l)})
\end{equation}

where $\mathbf{x}^{(l-1)}$ represents the output from the $(l-1)$-th layer, $\mathbf{W}^{(l)}$ is the weight matrix, $\mathbf{b}^{(l-1)}$ is the bias vector for $l$-th layer, and $\sigma(\cdot)$ is the activation function. Their ability to effectively model non-linear relationships makes MLPs well-suited for capturing the dynamics of complex systems. Consequently, they have become a primary choice as a functional approximation in the PINN frameworks.

Previous research has demonstrated the effectiveness of MLPs in solving inverse ECG problems \cite{xie_physics-constrained_2023}. However, it is found that the trainability of the EPDL introduces ineffective scaling or even degradation as the MLP network increases. As such, traditional PINNs, and more specifically, EP-DL frameworks, typically employ small and shallow neural networks with only 5 layers, limiting their ability to fully leverage the advantages of deeper architectures. %This presents a striking contrast to other applications of deep learning, where significantly deeper neural networks are commonly utilized to achieve superior performance. 
Moreover, conventional EP-DL approaches often face challenges with pathological initialization, where the initial training epochs produce an unbalanced loss with large magnitudes, resulting in unstable optimization and slower convergence. 
%these networks often suffer from a bad initialization issue, where the initial physics loss is excessively large, leading to slow training, model instability, or even failure to learn the correct physics \cite{mo_data-driven_2022,cuomo_scientific_2022}.
%Additionally, when increasing the depth and complexity of the FNNs, it is common that for PINNs, deeper networks tend to have higher error rates and fail to utilize the added layers effectively, limiting the model’s ability to learn deeper patterns \cite{berg_unified_2018}.

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{figures/resblock.png}
\caption{Adaptive residual block structure}
\label{resblock}
\end{figure}

To overcome the above limitations, our study innovatively introduces a novel adaptive residual block, specifically designed to address the problem of ineffective scaling and ill-posed initialization problem. %By introducing shortcut connections, residual blocks allow the input of a layer to skip one or more layers and add the input $x$ directly to the output of the residual block $F(x)$, which eventually constructs the output as $y=F(x)+x$ \cite{he_deep_2015}.
The architecture of the proposed adaptive residual block is shown in figure \ref{resblock}. Specifically, we defined a shortcut connection across stacked layers, allowing the input $x$ to flow directly to the output. The mathematical representation of adaptive residual block is defined as:

% \begin{align}
% \mathbf{h}^{(b)}_1 &= \sigma(\mathbf{W_1}^{(b)} \mathbf{x}^{(b)} + \mathbf{b_b}^{(b)})\\
% \mathbf{h}^{(b)}_2 &= \sigma(\mathbf{W_2}^{(b)} \mathbf{h_1} + \mathbf{b_2}^{(b)})\\
% \mathbf{x}^{(b+1)} &= \alpha^{(b)} \mathbf{h}^{(b)}_2 + (1 - \alpha^{(b)}) \mathbf{x}^{(b)}
% \end{align}

\begin{align}
\mathbf{h_1}^{(b)} &= \sigma(\mathbf{W_1}^{(b)} \mathbf{x}^{(b)} + \mathbf{b_1}^{(b)})\\
\mathbf{h_2}^{(b)} &= \sigma(\mathbf{W_2}^{(b)} \mathbf{h_1}^{(b)} + \mathbf{b_2}^{(b)})\\
\mathbf{x}^{(b+1)} &= \alpha^{(b)} \mathbf{h_2}^{(b)} + (1 - \alpha^{(b)}) \mathbf{x}^{(b)}
\end{align}

where $\mathbf{x}^{b}$ is defined as the input of the $b$-th adaptive residual block (Adap-ResBlock), $\mathbf{h_1}^{(b)}$ and $\mathbf{h_2}^{(b)}$ are the output of the hidden layers within the $b$-th Adap-ResBlock. $\mathbf{W}$'s and $\mathbf{b}$'s are the trainable neural net parameters. $\alpha$ is a hyperparameter that controls the proportion of the knowledge that directly inherited from the input $\mathbf{x}$.

%and the output of the Adaptive ResBlock $F(x)$ is equal to $\mathbf{h_2}$, and $\mathbf{x}^{l+1}$ is the output after the residual block. From the equations above, when $\alpha$ = 0, $\mathbf{x}^{(l+1)} = \mathbf{x}^{(l)}$, meaning that the model completely skip the residual block. In contrast, when $\alpha$ = 1, the model does not skip the residual block. Throughout the training process, $\alpha$ is initialized to $0$, thus allowing the network to effectively act as a shallow structure initially before gradually adjusting its complexity in accordance with the problem's nonlinearity.



To improve the explainability of the results, it is beneficial to determine the percentage of the input that flows directly to the output versus the percentage of the output contributed by the functional block. To ensure the contribution percentage 
$\alpha$ represents a meaningful proportion, it should be constrained between 0 and 1. This is achieved by introducing a trainable parameter 
$\alpha_T$ and applying a sigmoid function, which ensures $\alpha$ stays within the desired range:  %As such, it is essential to constrain the contribution percentage $\alpha$ between 0 and 1. This ensures that the parameter represents a meaningful proportion of the total contribution. To constrain $\alpha$ falls between 0 to 1, we introduce a trainable parameter $\alpha_T$. And then we apply a Sigmoid function to it so that $\alpha$ falls between 0 to 1:

%trainable parameter $\alpha$ as the coefficient of residual block output $F(x)$, and let $1-\alpha$ as the coefficient of input mapping $x$. By introducing this parameter $\alpha$, we were able to modulate the non-linearity within the residual block by adjusting the weight of input mapping $x$ and the residual block output $F(x)$ to the final output $y$. For better interpretability, to get the $\alpha$, we apply the sigmoid function to the original value $\alpha_T$ during training. The sigmoid function can be represented as:
\begin{equation*}
    \alpha = \frac{1}{1 + e^{-\alpha_T}}
\end{equation*}
%which allows us strictly limits $\alpha$'s value between 0 and 1 \cite{apicella_survey_2021}. 

By progressively deepening the network during training, these adaptive connections allow for an improved and more stable training process, making the network less susceptible to poor initialization and effectively mitigating the convergence issue. With the inclusion of adaptive residual blocks, we were able to add additional layers and neurons and further enhancing the model's ability to capture the complicated spatiotemporal dependencies in the HSP data. Specifically, the deeper architecture provides a greater capacity for feature extraction, while the increased number of neurons in each layer enhances the network's ability to learn richer representations at each level.

\begin{figure}[hb]
\centering
\includegraphics[width=3.5in]{figures/fnn.png}
\caption{FNN structure}
\label{fnn}
\end{figure}

The model employed in this study is a adaptive ResNet, integrated with adaptive residual blocks. The structure of our model is shown in figure \ref{fnn}. This architecture is designed to solve the inverse ECG problem, focusing on reconstructing the HSP using BSPM. The hyperbolic tangent (tanh) activation function was selected due to its effectiveness in training deep neural networks. Additionally, the model is trained with a custom loss function that incorporates physics-based constraints. A detailed description of the neural network’s architecture and the selection of its optimal structure will be provided in the following subsections.

\subsection{Numerical Differentiation on Spatiotemporal Domain}
For the AP model, there is a boundary condition to restrict the flow of electric current to remain confined within the heart's surface. A commonly applied method involves the use of the normal derivative operator for the potential distribution on the heart surface. The surface Laplacian of the boundary condition is usually calculated by the normal derivative of the heart surface potential. However, it focuses solely on the perpendicular component of the gradient, leaving out the tangential component along the surface. Consequently, this approach overlooks the interrelation between neighboring regions of the heart’s surface, which presents a challenge for achieving accurate modeling, particularly in high-dimensional contexts.

In the PINN training process, the partial derivative is critical for evaluating the residual loss of the differential equations at collocation points. For most PINN implementations, the partial derivative can be easily obtained by auto-differentiation (AD). This function is integrated into the deep learning training frameworks, when the PINN is higher order differentiable, it calculates the accurate derivative automatically during the backpropagation \cite{baydin_automatic_2018}. However, AD does not account for the local spatial structure, so it could not utilize the 3D geometric information. Moreover, when the amount of collocation points is insufficient, AD tends to cause the model overfiting to those specific locations, even though the training loss may be minimized, the model's accuracy may still be far from the true value. This is because AD computes the differential operators only at the specific collocation points, but when the neural network has excessive complexity, the loss function becomes under-constrained.

To address the aforementioned challenges, we employed numerical differentiation methods on the cardiac spatiotemporal domain, which enabled us to incorporate the heart geometric information into our model and, therefore, improved the reliability and robustness of our model. The methods we propose are elaborated as follows:

\textit{1) Spatial Laplacian:} As the surface Laplacian does not account for the spatial correlations or the intricate geometries inherent in our data, to provide better spatial regularization to our model, we replace the surface Laplacian with the spatial Laplacian $\Delta_{s}$. The $\Delta_{s}$ is a matrix consisting of the Laplacian of each mesh node, and the Laplacian was computed as a weighted sum of interpolated values from the neighboring nodes \cite{yao_physics-driven_2016}.

\begin{figure}[hb]
\centering
\includegraphics[width=2.5in]{figures/mesh.png}
\caption{3D triangle mesh on human heart surface}
\label{fig:laplacian}
\end{figure}

Specifically, we discretized the cardiac surface into irregular triangle meshes, as shown in figure \ref{fig:laplacian}, which better conforms to the 3D heart geometry. Let $u_{j’}$ be the value of our function $u(s, t)$ at node $s_{j}’$, and $d_{ij}$ be the distance from node $s_i$ to $s_j$, and $\overline{d}_{j}$ be the average distance between all the neighbor points and $s_2$. Using the linear interpolation, $u_{j'}$ can be expressed as:
\begin{equation}
    u_{j'} = u_{i} + \frac{\overline{d}_{j}}{d_{ij}} (u_{j}-u_{i})
\end{equation}

For the triangles where $s_i$ is included as the vertice, we use $s_{j}'$ as the neighbor points. Then, the Laplacian of $u_i$ at $s_i$ is:
\begin{align}
    \Delta_{s} (u_i) &= \frac{4}{\overline{d_i}^2} \left( \frac{1}{n_i} \sum_{j=1}^{n_i} u_{j}' - u_i \right)\\
    &= \frac{4}{\overline{d_i}} \left( \frac{1}{n_i} \sum_{j=1}^{n_i} \frac{u_j}{d_{ij}} - \left( \frac{1}{d_i} \right) u_i \right)
\end{align}

Therefore, the elements in the spacial Laplacian matrix $\Delta_{s}$ can be denoted as:
\begin{align}
    \Delta_s = 
    \begin{cases}
    -\frac{4}{\overline{d_i}} \left( \frac{1}{d_i} \right), & \text{if } i = j \\
    \frac{4}{\overline{d_i}} \frac{1}{n_i d_{ij}}, & \text{if } i \neq j, p_j \in \text{neighborhood of } p_i \\
    0, & \text{otherwise}
    \end{cases}
\end{align}

\textit{2) Numerical Differentiation:} As mentioned above, AD could not incorporate the geometric information, and it expects a large set of collocation points to ensure high accuracy. Corresponding to the AD method, an alternative approach to obtain the partial derivative is numerical differentiation (ND), which is a well-established technique in the fields of scientific computing and computational physics \cite{ahnert_numerical_2007}. ND, in particular, the finite-difference method, approximates the derivative of a function that the values on a fixed grid. It uses the local numerical schemes and computes the derivative by canceling out the leading error terms of Taylor-series expansions. As a result, ND enables the model to learn spatial patterns and provides more robust results with respect to the number of collocation points. 

The accuracy of ND is determined by the number of neighbor points used for the Taylor-series expansion, the more neighbor points will give the higher order of the error terms and, therefore, higher accuracy of the approximation. But more neighbor points also increase the computation effort. In fact, the commonly used second-order ND is less accurate than AD, it introduces errors and may not fully capture the complexity of certain physical systems, especially in scenarios like cardiac electrophysiology that require high precision. In order to balance the precision requirement of the approximation and the computation constraint, in our research, we implemented the finite difference with fourth-order accuracy (4th-ND).

\begin{figure}[!t]
\centering
\includegraphics[width=2.8in]{figures/4thND.png}
\caption{Schematic of point location for 4th-ND calculation at an interior point when $t=t_0$}
\label{fig:4th-nd}
\end{figure}

Given our function $u(t)$ and fixed time interval $\tau$, for 4th-ND, at time $t$, we need to consider five adjacent points, $u_{t-2}, u_{t-1}, u_{t}, u_{t+1}$ and $u_{t+2}$, where  $u_{t}$ is the current central point, with $u_{t-2}$ and $u_{t-1}$ positioned to the left of $u_{t}$, $u_{t+1}$ and $u_{t+2}$ positioned to the right of $u_{t}$, and the time interval between each neighbor points is $\tau$, as illustrated in the figure \ref{fig:4th-nd}. For the internal points, we adopted the central difference method, namely approximate the derivative of the current point using the neighbor points on both sides equally, so we placed the five points at $t-2$, $t-1$, $t$, $t+1$, $t+2$ respectfully. Then, according to the Taylor-series expansion, the fifth-order expansion polynomials of the five points are as follows:

\begin{align}
    u_{t-2} &= u_{t} + \tau \frac{\partial u_{t}}{\partial t} 
    + \frac{\tau^2}{2!} \frac{\partial^2 u_{t}}{\partial t^2} 
    + \frac{\tau^3}{3!} \frac{\partial^3 u_{t}}{\partial t^3} + \frac{\tau^4}{4!} \frac{\partial^4 u_{t}}{\partial t^4} 
    + O(\tau^5)\\
    u_{t-1} &= u_{t} + 2\tau \frac{\partial u_{t}}{\partial t} 
    + \frac{(2\tau)^2}{2!} \frac{\partial^2 u_{t}}{\partial t^2} 
    + \frac{(2\tau)^3}{3!} \frac{\partial^3 u_{t}}{\partial t^3} \notag \\
    &\quad + \frac{(2\tau)^4}{4!} \frac{\partial^4 u_{t}}{\partial t^4} 
    + O(\tau^5)\\
    u_{t+1} &= u_{t} - \tau \frac{\partial u_{t}}{\partial t} 
    + \frac{\tau^2}{2!} \frac{\partial^2 u_{t}}{\partial t^2} 
    - \frac{\tau^3}{3!} \frac{\partial^3 u_{t}}{\partial t^3} + \frac{\tau^4}{4!} \frac{\partial^4 u_{t}}{\partial t^4} 
    + O(\tau^5)\\
    u_{t+2} &= u_{t} - 2\tau \frac{\partial u_{t}}{\partial t} 
    + \frac{(2\tau)^2}{2!} \frac{\partial^2 u_{t}}{\partial t^2} 
    - \frac{(2\tau)^3}{3!} \frac{\partial^3 u_{t}}{\partial t^3} \notag \\
    &\quad + \frac{(2\tau)^4}{4!} \frac{\partial^4 u_{t}}{\partial t^4} 
    + O(\tau^5)
\end{align}

where the value of $u_{t}$, $u_{t-2}$, $u_{t-1}$, $u_{t+1}$ and $u_{t+2}$ is known. Therefore, we could solve this system of equations and result in the approximation for the derivatives of $u$ with respect to the time $t$, denoted as $u_{t}’$:

\begin{align}
    u_{t}'\approx \frac{u_{t-2} - 8u_{t-1} + 8u_{t+1} - u_{t+2}}{12\tau}
\end{align}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{figures/4thND2.png}
\caption{Schematic of point location for 4th-ND calculation at boundary}
\label{fig:4th-nd2}
\end{figure}

For the boundary points, where we cannot use points on both sides equally, the derivatives are computed similarly but use the five nearest neighboring points instead. As shown in figure \ref{fig:4th-nd2}, let $u_{0}$ and $u_{1}$ be the first two points with $u_{2}, u_{3}, u_{4}$ as their neighbor points, $u_{T-1}$ and $u_{T}$ be the last two points with $u_{T-2}, u_{T-3}, u_{T-4}$ as their neighbor points, their derivatives are computed as:

\begin{align}
    u_{0}' &\approx \frac{-25u_{0} + 48u_{1} - 36u_{2} + 16u_{3} - 3u_{4}}{12\tau}\\
    u_{1}' &\approx \frac{-3u_{0} - 10u_{1} + 18u_{2} - 6u_{3} + u_{4}}{12\tau}\\
    u_{T-1}'&\approx \frac{-u_{T-4} + 6u_{T-3} - 18u_{T-2} + 10u_{T-1} + 3u_{T}}{12\tau}\\
    u_{T}' &\approx \frac{3u_{T-4} - 16u_{T-3} + 36u_{T-2} - 48u_{T-1} + 25u_{T}}{12\tau}
\end{align}

\subsection{Physics Awareness Approach}
Incorporating physics knowledge into the neural network training process is a critical part of a PINN model. In our proposed framework for solving the inverse ECG problem, we integrated the AP model into our PINN through a dedicated EP awareness loss function that penalizes deviations from the AP model equations. This customized loss function enables the model to be trained under both data-driven constraints and physics law constraints, which leads to the correct spatiotemporal behavior of the cardiac electrical dynamics and ensures the model predictions adhere to the physiological principles of cardiac electrophysiology.

Specifically, for our PINN model, we denote $s$ as the 3D space coordinates and $t$ as the time coordinate, the input of the network consists of the spatiotemporal coordinates $[s, t]$ of the dynamic system,  and the prediction of HSP $u(s, t)$ and recovery current $v(s, t)$ are the output. The EP awareness loss function is defined through the following formula:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{\text{D}} + \lambda \cdot \mathcal{L}_{\text{Ep}}
\end{equation}
where $\mathcal{L}$ represents the total loss,$\mathcal{L}_{\text{D}}$ and $\mathcal{L}_{\text{EP}}$ represent the data-driven loss and EP awareness loss respectfully, $\lambda$ is an adjustable weighting factor to regulate the intensity of EP awareness loss. 

\textit{1) Data-driven Loss:} The data-driven loss $\mathcal{L}_{\text{D}}$ is calculated by measuring the discrepancy between the model predicted HSP $\hat{u}(s, t)$ and the actual sensor measurements. In our research, BSP is provided as the sensor measurements $y(s, t)$, and we use a transfer matrix $R$ to map our $\hat{u}(s, t)$ to the predicted BSP $R\hat{u}(s, t)$. The derivation of transfer matrix $R$ can be referred to \cite{yao_spatiotemporal_2020,barr_relating_1977}.  Therefore, the data-driven loss is computed as the mean squared error of total number of points $N$ between the measured BSP $y(s, t)$ and the predicted BSP $R\hat{u}(s, t)$, which is defined as:
\begin{equation}
    \mathcal{L}_{\text{D}} = \frac{1}{N} \sum_{t} \sum_{s} \| y(s,t) - R\hat{u}(s,t) \|^2
\end{equation}

\textit{2) EP Awareness Loss:} To further improve the accuracy and stability of our model predictions, we incorporate physics-based constraints at randomly sampled spatiotemporal collocation points, selected from points within the spatial boundaries of the 3D heart geometry and the temporal range of the cardiac cycle. The physics constraint is derived by minimizing PDEs residuals of the AP model. residuals. Additionally, as described in the previous subsection, we strengthen the geometry information provided to the model by replacing the surface Laplacian with the spatial Laplacian and utilizing the 4th-ND scheme to compute first-order temporal derivatives. The physics constraint residuals are formulated as:

\begin{align}
    r_u(s, t) &= \frac{\partial \hat{u}}{\partial t} - D \cdot\Delta_{s} \hat{u} - k_r \hat{u}(1 - \hat{u})(\hat{u} - a) + \hat{u} \hat{v}\\
    r_v(s, t) &= \frac{\partial \hat{v}}{\partial t} - \varepsilon(\hat{u}, \hat{v})(-\hat{v} - k_r \hat{u} (\hat{u} - a - 1))
\end{align}

Let $N$ represent the number of collocation points, as we need to minimize the AP model residuals for these collocation points, therefore our EP awareness loss can be formulated as:

\begin{equation}
    \mathcal{L}_{\text{Ep}} = \frac{1}{N} \sum_{i=1}^{N} \left[ r_u(s_i, t_i)^2 + r_v(s_i, t_i)^2 \right]
\end{equation}

By integrating the data-driven loss with the EP awareness loss, we formulate a custom loss function that embeds physical prior knowledge. This combined loss function is used to train our FNN, enhancing the model’s prediction accuracy and improving its generalization capability.

